Who Verifies the Verifiers? Accountable Semantic Consensus for AI-Mediated Web Information Verification

Large language models (LLMs) increasingly decide whether Web evidence supports online claims, often by voting over several assessors whose errors are presumed independent and benign. On the open Web, retrieved pages can steer the assessors that read them, and assessors from one model family fail together. We prove that even for independent assessors whose every output sequence is possible on both valid and invalid claims, any protocol that decides only from their outputs and always reaches an agreed verdict never rejects invalid claims or rejects valid ones with positive probability. We present Astral, which pins all assessors to one committed snapshot of the Web evidence. With up to f assessors faulty, Astral accepts a verdict only when 2f+1 assessors attest to it above a confidence threshold and no signed challenge stands. On five public benchmarks with two of seven assessors adversarial, Astral lowers pooled attack success to 21.5-53.1%, against 54.7-77.8% for majority voting. The cost is coverage, as without attack 16.0-61.7% of claims receive a binary verdict and the rest are disputed for audit. Our code runs at https://anonymous.4open.science/r/Astral-55F1.

==> tables/evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

The evaluation follows the three research questions of \S\ref{sec:introduction}.
RQ1 measures how accurately each aggregation rule decides benign Web claims (\S\ref{sec:eval:rq1}).
RQ2 measures how fast integrity degrades under adversarial assessors  (\S\ref{sec:eval:rq2}).
RQ3 measures what the challenge path, the bound, and assessor diversity contribute and what they cost (\S\ref{sec:eval:rq3}).

\subsection{Setup}\label{sec:eval:setup}

\leadtag{Public benchmarks}{tagsetup}{Tables~\ref{tab:astral_main_part1} and~\ref{tab:astral_main_part2} use fixed evaluation splits with published evidence and labels.}
Table~\ref{tab:astral_main_part1} covers AVeriTeC ($N{=}500$), Climate-FEVER ($N{=}1{,}535$), and FEVER ($N{=}15{,}935$); Table~\ref{tab:astral_main_part2} covers PUBHEALTH ($N{=}1{,}220$) and SciFact ($N{=}300$). Here $N$ is the number of claims in the fixed split used by the table, not the number of protocol trials. AVeriTeC and FEVER contain general fact-checking claims, Climate-FEVER contains climate claims, PUBHEALTH contains public-health claims, and SciFact contains scientific claims paired with abstracts. We replay each claim with its released evidence and ground-truth label; no benchmark claim, evidence item, or label is generated or rewritten by an LLM.

\leadtag{Synthetic and live cohorts}{tagsetup}{We use two additional cohorts to test controlled mechanisms and mutable evidence.}
Multi-source fact verification (MFV) pairs 100 synthetic claims over five topics with three to five evidence excerpts each, half supported and half refuted, with difficulty set by how consistent the excerpts are.
A live cohort of 80 vulnerability claims takes evidence from the NVD Web API, 40 for real \texttt{CRITICAL}-severity CVEs and 40 for fabricated ones.
Two non-Web domains (code patching and log auditing) appear in \textbf{Appendix~\ref{app:extra}}.

\leadtag{Assessors and harness}{tagsetup}{Committees of $n \in \{7, 13, 31, 67, 100\}$ assessors with $f = \lfloor (n-1)/3 \rfloor$ draw on seven model families, four of which form the $n{=}7$ committee (\textbf{Appendix~\ref{app:extra}}).}
For $n \geq 31$ the committee cycles over the seven families, so the number of independent sources stays at seven.
The SciFact and FEVER runs use a separate $n{=}7$ committee with one model from each of seven families (\Cref{tab:realbench}).
We use $k = 2f{+}1$, $\tau = 0.7$, and seed 42, with five-seed validation in \textbf{Appendix~\ref{app:multiseed}}.
API models decode greedily, local models use temperature 0.01, and each assessor's response to a claim is cached once and reused across protocols.
L2 and L3 are simulated in logical rounds on top of a deterministic L1 stub after GST, so $\Delta$, $W(v)$, $T_{\mathit{infer}}$, $T_{\mathit{DA}}$, and $T_{\mathit{arb}}$ take no wall-clock values.
The challenge window is a single round.
In it, every honest assessor whose $\vinfer$ label is $\mathsf{REJECT}$ attempts to file one counter, and a counter enters triage only if it passes \texttt{VerifyCounterStruct}.
The $m$ checkers of \S\ref{sec:design:probability} are therefore the honest assessors ($n{-}f$ in attack trials and all $n$ in benign trials), and each checker's detection outcome is its Phase~\textcircled{1} label.
Each assessor casts one triage vote, and a counter with fewer than $2f{+}1$ \texttt{COUNTER\_REJECT} votes sends the decision to \texttt{DISPUTED}.
This rule replaces the $T_{\mathit{arb}}$ fallback in the simulation.
Diversity comes from committee composition, and the diversity predicate is left unchecked at attestation time.

\leadtag{Adversarial assessors}{tagthreat}{In attack trials, $f$ assessors are Byzantine and attest with confidence 0.95.}
Prompt or tool injection (A1)~\cite{promptinjection} feeds them injected instructions that steer them to the wrong verdict.
In a fabricated proposal (A2), a Byzantine leader proposes a plausible false verdict.
Evidence truncation (A3) has them drop 30\% of the evidence and endorse the incomplete decision object.
Model-aware corruption (A4) places the $f$ Byzantine slots on the assessors that reject most reliably and leaves the weakest models honest.
Counter-spam (A5) files one structurally valid but vacuous counter per Byzantine assessor and window.

\leadtag{Baselines and metrics}{tagsetup}{We compare against majority voting (MV) over the assessors' labels and against CP-WBFT~\cite{cpwbft}, which probes confidence and refines labels with confidence-weighted aggregation.}
L1-BFT, which orders verdicts without semantic checks, and an oracle with a perfect $\vinfer$ bound the range.
\astral-NoCh drops the challenge window, \astral-NoDiv uses one backend for all assessors, and Simple Threshold accepts on one assessor's confidence.
In Tables~\ref{tab:astral_main_part1} and~\ref{tab:astral_main_part2}, ``Single-model (avg.)'' averages seven independent single-backend runs, ``w/o Challenge'' is \astral-NoCh, and ``Simple-Thr.'' is the single-assessor threshold baseline.
For Tables~\ref{tab:astral_main_part1} and~\ref{tab:astral_main_part2}, the semantic correctness success rate (SCSR) is the fraction of benign trials whose final binary decision matches the ground-truth label. Coverage (Cov.) is the fraction of benign trials that end in a binary \texttt{ACCEPT} or \texttt{REJECT}, rather than \texttt{DISPUTED}. Each A1--A4 column is the attack success rate for that attack: a refuted claim counts as a success only when the final output is \texttt{ACCEPT}; a \texttt{DISPUTED} output is safe but reduces coverage. The pooled ASR aggregates accepted refuted claims over all four attacks, and Disp. is the fraction of attacked trials that end in \texttt{DISPUTED}. Brackets report Clopper--Pearson 95\% confidence intervals for pooled ASR; the other entries are point estimates.

\subsection{RQ1: Reliability under Benign Disagreement}\label{sec:eval:rq1}

\input{tables/tab_realbench}

Without adversaries, every semantic aggregator decides most Web claims correctly (\Cref{tab:realbench}).
On SciFact, MV and CP-WBFT reach 92.5\% and 92.0\% SCSR and \astral reaches 86.5\%.
On FEVER, the three reach 96.5\%, 97.0\%, and 94.5\%.
The quorum is not the source of this gap.
\astral-NoCh keeps the $2f{+}1$ confidence-filtered quorum, drops the challenge window, and reaches 93.5\% and 96.5\%.
The 2.0 to 7.0 points that full \astral loses relative to \astral-NoCh are consistent with the challenge path, in which an honest assessor that rejects a supported claim files a counter and an undismissed counter sends the decision to \texttt{DISPUTED}.
On the synthetic suite, \astral's SCSR falls from 92.9\% at $n{=}7$ to 82.4\% at $n \geq 13$, while MV and CP-WBFT stay near 94\% (\textbf{Appendix~\ref{app:extra}}).

\takeawaybox{Under benign disagreement, \astral's confidence-filtered quorum decides public Web claims as accurately as label aggregation, and adding the challenge window coincides with a loss of 2.0 to 7.0 points of benign correctness.}

\subsection{RQ2: Robustness to Adversarial Assessors and Web Evidence}\label{sec:eval:rq2}

\input{tables/www_mfv_asr}

\leadtag{Adversarial assessors}{tagthreat}{With two of seven assessors adversarial, \astral accepts no refuted SciFact claim and 0.5\% of refuted FEVER claims, against 7.8\% and 4.0\% for MV and 20.2\% and 3.2\% for CP-WBFT (\Cref{tab:realbench}).}
L1-BFT accepts every refuted claim, which shows that ordering without a semantic check offers no protection.
A single assessor with the same confidence threshold (Simple Threshold) already reaches 3.0\% and 2.8\%, so the confidence filter accounts for much of the gap to label aggregation.
The $2f{+}1$ quorum lowers attack success to 1.8\% and 2.5\% (\astral-NoCh), and the challenge window lowers it to 0.0\% and 0.5\% while attaching a signed record to every decision.
CP-WBFT is weakest where one confident assessor can move the others.
On MFV it accepts 20--36\% of refuted multi-source claims, because its refinement step lets a single assessor reporting confidence 0.95 pull honest assessors to its label (\Cref{tab:mfv_asr}A).
\astral keeps MFV attack success at 2--4\%.

\leadtag{Correlated assessors}{tagsemantic}{Growing the committee by replicating the same seven families adds assessors that err together.}
Under model-aware corruption, MV rises from 6\% to 10\% and CP-WBFT from 28\% to 36--38\% on MFV as $n$ grows, while \astral stays at 0--4\% (\Cref{tab:mfv_asr}B).
In the non-Web domains the same replication raises MV's attack success to 88\% on log auditing at $n \geq 13$ (\textbf{Appendix~\ref{app:extra}}).
% Required in the paper preamble: \usepackage{booktabs}\usepackage{colortbl}
% If your template already loads xcolor, do not load it again with new options.
\begin{table*}[t]
\centering
\caption{Main results on AVeriTeC, Climate-FEVER, and FEVER using seven open-weight assessors. $N$ is the claim count in the fixed evaluation split. SCSR and Cov. are clean metrics; A1--A4 are attack success rates, and pooled ASR aggregates the four attacks.}
\label{tab:astral_main_part1}
\begingroup
\setlength{\tabcolsep}{5.3pt}
\renewcommand{\arraystretch}{1.0}
\fontsize{11}{13}\selectfont
\newcommand{\ASRCI}[3]{\mbox{#1\,{\fontsize{8.0}{9.3}\selectfont\color[gray]{0.42}[#2,#3]}}}
\begin{tabular}{l*{8}{r}}
\toprule
& \multicolumn{2}{c}{\textbf{Clean}} & \multicolumn{6}{c}{\textbf{Byzantine attacks (\%)}} \\
\cmidrule(lr){2-3}\cmidrule(l){4-9}
\textbf{Method} & \textbf{SCSR}$\uparrow$ & \textbf{Cov.}$\uparrow$ & \textbf{A1}$\downarrow$ & \textbf{A2}$\downarrow$ & \textbf{A3}$\downarrow$ & \textbf{A4}$\downarrow$ & \textbf{ASR}$\downarrow$ & \textbf{Disp.}$^{\dagger}$ \\
\midrule
\rowcolor[RGB]{240,240,240}\multicolumn{9}{c}{\rule{0pt}{12.5pt}\textbf{AVeriTeC}\ {\normalfont\color[gray]{0.42}($N=500$)}} \\
L1-BFT & 24.4 & \textbf{100.0} & 100.0 & 100.0 & 100.0 & 100.0 & \ASRCI{100.0}{99.8}{100.0} & 0.0 \\
MV & \textbf{88.2} & \textbf{100.0} & 96.6 & 17.5 & 26.7 & 100.0 & \ASRCI{60.2}{57.7}{62.7} & 0.0 \\
CP-WBFT & 50.6 & \textbf{100.0} & 97.6 & 50.3 & 51.9 & 100.0 & \ASRCI{74.9}{72.7}{77.1} & 0.0 \\
Simple-Thr. & 75.6 & \textbf{100.0} & 73.0 & 40.5 & 45.0 & 85.4 & \ASRCI{61.0}{58.5}{63.4} & 0.0 \\
\cmidrule(lr){1-9}
Single-model (avg.) & 77.6 & 25.9 & 57.1 & 15.8 & 20.4 & 57.1 & 37.6 & 17.3 \\
w/o Challenge & 86.0 & 10.8 & 64.6 & 3.4 & 9.5 & 99.7 & \ASRCI{44.3}{41.8}{46.9} & 0.0 \\
\rowcolor[RGB]{229,236,250} \textbf{ASTRAL} & 82.6 & 7.0 & \textbf{27.2} & \textbf{1.6} & \textbf{6.1} & \textbf{51.1} & \ASRCI{\textbf{21.5}}{19.4}{23.7} & 50.5 \\
\addlinespace[3pt]
\rowcolor[RGB]{240,240,240}\multicolumn{9}{c}{\rule{0pt}{12.5pt}\textbf{Climate-FEVER}\ {\normalfont\color[gray]{0.42}($N=1{,}535$)}} \\
L1-BFT & 42.6 & \textbf{100.0} & 100.0 & 100.0 & 100.0 & 100.0 & \ASRCI{100.0}{99.9}{100.0} & 0.0 \\
MV & \textbf{70.4} & \textbf{100.0} & 99.3 & 42.3 & 45.1 & 100.0 & \ASRCI{71.7}{70.2}{73.2} & 0.0 \\
CP-WBFT & 46.3 & \textbf{100.0} & 99.3 & 67.4 & 74.2 & 100.0 & \ASRCI{85.2}{84.0}{86.4} & 0.0 \\
Simple-Thr. & 61.8 & \textbf{100.0} & 77.8 & 52.9 & 47.3 & 90.8 & \ASRCI{67.2}{65.6}{68.7} & 0.0 \\
\cmidrule(lr){1-9}
Single-model (avg.) & 62.1 & 38.0 & 68.5 & 29.0 & 29.6 & \textbf{68.5} & 48.9 & 9.6 \\
w/o Challenge & 67.9 & 16.7 & 84.3 & 14.9 & 14.8 & 100.0 & \ASRCI{53.5}{51.8}{55.1} & 0.0 \\
\rowcolor[RGB]{229,236,250} \textbf{ASTRAL} & 65.1 & 11.7 & \textbf{61.1} & \textbf{11.4} & \textbf{11.7} & 87.9 & \ASRCI{\textbf{43.0}}{41.3}{44.6} & 26.7 \\
\addlinespace[3pt]
\rowcolor[RGB]{240,240,240}\multicolumn{9}{c}{\rule{0pt}{12.5pt}\textbf{FEVER}\ {\normalfont\color[gray]{0.42}($N=15{,}935$)}} \\
L1-BFT & 29.1 & \textbf{100.0} & 100.0 & 100.0 & 100.0 & 100.0 & \ASRCI{100.0}{100.0}{100.0} & 0.0 \\
MV & 83.0 & \textbf{100.0} & 99.5 & 54.0 & 47.6 & 100.0 & \ASRCI{75.3}{74.9}{75.7} & 0.0 \\
CP-WBFT & 44.3 & \textbf{100.0} & 99.7 & 66.5 & 57.8 & 100.0 & \ASRCI{81.0}{80.6}{81.3} & 0.0 \\
Simple-Thr. & 67.5 & \textbf{100.0} & 75.7 & 52.3 & 49.6 & 91.3 & \ASRCI{67.2}{66.8}{67.6} & 0.0 \\
\cmidrule(lr){1-9}
Single-model (avg.) & 67.7 & 44.0 & 66.3 & 33.3 & 29.5 & \textbf{66.3} & 48.9 & 14.0 \\
w/o Challenge & \textbf{84.5} & 24.3 & 83.1 & 20.6 & 15.1 & 100.0 & \ASRCI{54.7}{54.2}{55.2} & 0.0 \\
\rowcolor[RGB]{229,236,250} \textbf{ASTRAL} & 81.5 & 17.6 & \textbf{53.4} & \textbf{15.0} & \textbf{12.4} & 67.2 & \ASRCI{\textbf{37.0}}{36.6}{37.4} & 31.9 \\
\bottomrule
\end{tabular}
\endgroup
\vspace{3pt}
\parbox{0.96\textwidth}{\footnotesize \emph{Notes.} All metrics in \%. $\uparrow$/$\downarrow$: higher/lower is better; bold: best within each dataset (ties included). $^{\dagger}$Disp. is the disputed-output rate (no fixed preference). ASR pools A1--A4; brackets give Clopper--Pearson 95\% CIs. Single-model (avg.) averages seven single-backend runs (CI unavailable); w/o Challenge removes challenge.}
\end{table*}

% Required in the paper preamble: \usepackage{booktabs}\usepackage{colortbl}
% If your template already loads xcolor, do not load it again with new options.
Table~\ref{tab:astral_main_part2} applies the same protocol and metric definitions to the public-health and scientific-claim splits. This makes the comparison across Tables~\ref{tab:astral_main_part1} and~\ref{tab:astral_main_part2} like-for-like: the only change is the benchmark and its fixed claim split.

\begin{table*}[t]
\centering
\caption{Main results on PUBHEALTH and SciFact using seven open-weight assessors. $N$ is the claim count in the fixed evaluation split. Clean and attack metrics use the definitions above; pooled ASR aggregates A1--A4.}
\label{tab:astral_main_part2}
\begingroup
\setlength{\tabcolsep}{5.3pt}
\renewcommand{\arraystretch}{1.0}
\fontsize{11}{13}\selectfont
\newcommand{\ASRCI}[3]{\mbox{#1\,{\fontsize{8.0}{9.3}\selectfont\color[gray]{0.42}[#2,#3]}}}
\begin{tabular}{l*{8}{r}}
\toprule
& \multicolumn{2}{c}{\textbf{Clean}} & \multicolumn{6}{c}{\textbf{Byzantine attacks (\%)}} \\
\cmidrule(lr){2-3}\cmidrule(l){4-9}
\textbf{Method} & \textbf{SCSR}$\uparrow$ & \textbf{Cov.}$\uparrow$ & \textbf{A1}$\downarrow$ & \textbf{A2}$\downarrow$ & \textbf{A3}$\downarrow$ & \textbf{A4}$\downarrow$ & \textbf{ASR}$\downarrow$ & \textbf{Disp.}$^{\dagger}$ \\
\midrule
\rowcolor[RGB]{240,240,240}\multicolumn{9}{c}{\rule{0pt}{12.5pt}\textbf{PUBHEALTH}\ {\normalfont\color[gray]{0.42}($N=1{,}220$)}} \\
L1-BFT & 51.6 & \textbf{100.0} & 100.0 & 100.0 & 100.0 & 100.0 & \ASRCI{100.0}{99.8}{100.0} & 0.0 \\
MV & 62.8 & \textbf{100.0} & 97.0 & 7.8 & 14.2 & 100.0 & \ASRCI{54.7}{52.7}{56.8} & 0.0 \\
CP-WBFT & \textbf{72.6} & \textbf{100.0} & 96.4 & 35.5 & 51.3 & 100.0 & \ASRCI{70.8}{68.9}{72.6} & 0.0 \\
Simple-Thr. & 62.5 & \textbf{100.0} & 70.9 & 30.8 & 43.5 & 83.1 & \ASRCI{57.1}{55.0}{59.1} & 0.0 \\
\cmidrule(lr){1-9}
Single-model (avg.) & 63.2 & 22.5 & 57.9 & 8.0 & 12.9 & \textbf{57.9} & \textbf{34.2} & 5.9 \\
w/o Challenge & 55.5 & 7.7 & 66.5 & \textbf{2.4} & 4.1 & 100.0 & \ASRCI{43.2}{41.2}{45.3} & 0.0 \\
\rowcolor[RGB]{229,236,250} \textbf{ASTRAL} & 54.6 & 6.8 & \textbf{45.7} & \textbf{2.4} & \textbf{3.7} & 92.6 & \ASRCI{36.1}{34.1}{38.1} & 16.8 \\
\addlinespace[3pt]
\rowcolor[RGB]{240,240,240}\multicolumn{9}{c}{\rule{0pt}{12.5pt}\textbf{SciFact}\ {\normalfont\color[gray]{0.42}($N=300$)}} \\
L1-BFT & 41.3 & \textbf{100.0} & 100.0 & 100.0 & 100.0 & 100.0 & \ASRCI{100.0}{99.5}{100.0} & 0.0 \\
MV & 63.7 & \textbf{100.0} & 99.4 & 71.0 & 40.9 & 100.0 & \ASRCI{77.8}{74.6}{80.9} & 0.0 \\
CP-WBFT & 42.0 & \textbf{100.0} & 97.2 & 86.9 & 56.8 & 100.0 & \ASRCI{85.2}{82.4}{87.8} & 0.0 \\
Simple-Thr. & 60.7 & \textbf{100.0} & 82.4 & 59.1 & 50.6 & 94.3 & \ASRCI{71.6}{68.1}{74.9} & 0.0 \\
\cmidrule(lr){1-9}
Single-model (avg.) & 58.1 & 53.0 & 72.5 & 45.7 & 27.8 & \textbf{72.5} & 54.6 & 7.5 \\
w/o Challenge & \textbf{70.0} & 33.3 & 90.9 & 41.5 & 11.4 & 100.0 & \ASRCI{60.9}{57.2}{64.6} & 0.0 \\
\rowcolor[RGB]{229,236,250} \textbf{ASTRAL} & 69.7 & 30.3 & \textbf{72.2} & \textbf{36.4} & \textbf{10.2} & 93.8 & \ASRCI{\textbf{53.1}}{49.4}{56.9} & 16.5 \\
\bottomrule
\end{tabular}
\endgroup
\vspace{3pt}
\parbox{0.96\textwidth}{\footnotesize \emph{Notes.} All metrics in \%. $\uparrow$/$\downarrow$: higher/lower is better; bold: best within each dataset (ties included). $^{\dagger}$Disp. is the disputed-output rate (no fixed preference). ASR pools A1--A4; brackets give Clopper--Pearson 95\% CIs. Single-model (avg.) averages seven single-backend runs (CI unavailable); w/o Challenge removes challenge.}
\end{table*}

\leadtag{Manipulated Web evidence}{tagthreat}{This study perturbs the retrieved Web evidence instead of the assessors.}

\leadtag{Live Web evidence}{tagsemantic}{On the 80 live vulnerability claims at $n{=}7$, \astral supports 39 of 40 real CVEs (97.5\%, 95\% CI [86.8, 99.9]) and rejects all 40 fabricated ones, both without attack and under A1.}
With one assessor degraded to reject conservatively, it supports 38 of 40 real CVEs without attack and 39 of 40 under A1, and it still accepts no fabricated CVE.

\takeawaybox{When a minority of assessors is adversarial or correlated, label aggregation turns their errors into accepted Web verdicts, while \astral keeps attack success at 0.0--4.0\% across public and multi-source claims.}

\subsection{RQ3: Accountability, Diversity, and Cost}\label{sec:eval:rq3}

\begin{table}[t]
\centering
\caption{Assessor correlation on MFV ($\tau{=}0.7$), 50 trials per configuration. $k_h$ is the number of honest attesters in each calibration configuration.}\label{tab:rho}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Diversity configuration} & \textbf{$k_h$} & \textbf{$\Pr[\cap A_i]$} & \textbf{$\epsilon^{k_h}$} & \textbf{$\rho_{k_h}$} \\
\midrule
Same model family      & 2 & $2.0 \times 10^{-2}$ & $4.0 \times 10^{-4}$ & 50.0 \\
Mixed 2 families       & 2 & $2.0 \times 10^{-2}$ & $9.0 \times 10^{-4}$ & 22.2 \\
Mixed 3 families       & \astralsoft{3} & \astralsoft{$0$} & \astralsoft{$3.7 \times 10^{-5}$} & \astralsoft{0.0} \\
Full diversity (4+)    & \astralcell{4} & \astralcell{$0$} & \astralcell{$1.5 \times 10^{-6}$} & \astralcell{0.0} \\
\bottomrule
\end{tabular}
}
\end{table}

\leadtag{Diversity and the bound}{tagsemantic}{Assessor diversity determines how tight the residual-risk bound is, as shown in the correlation analysis below.}
A committee from one model family produced one joint false acceptance in 50 trials, which gives $\rho_{k_h} = 50$.
A single event leaves this estimate with a wide interval.
Two families also produced one joint false acceptance ($\rho_{k_h} = 22.2$), and three or more families produced none (95\% upper bound 0.06).
These rates are joint false-acceptance rates without the challenge factor of \Cref{eq:delta}.
Counters are filed in 56.7--59.0\% of attack trials (the accountability table in Appendix~\ref{app:extra}), which estimates $p_{\mathit{ch}}$ unconditionally.
The bound uses $p_{\mathit{ch}}$ conditioned on all honest attesters having falsely accepted, which can be lower, so we do not evaluate the bound end to end.
In the layer ablation, attestation alone lowers MFV attack success from 100\% to 6\% under A2 and the challenge window lowers it to 2\% (\textbf{Appendix~\ref{app:extra}}).
\astral-NoDiv reaches the same 2\%, but its single-family correlation factor of 50 loosens the bound accordingly.

\leadtag{Accountability}{tagdefense}{The challenge path turns disagreement into an attributable record instead of a silent label.}
At $n{=}7$ under attacks A1--A4, counters are filed in 56.7--59.0\% of trials, $\crqc$ resolution occurs in 5.0--8.9\%, and 53.8--55.7\% of decisions end as \texttt{DISPUTED}.
The Byzantine-detection rate is 58.3\% at $n{=}7$ and 67.0\% at $n{=}31$ (\Cref{tab:protocol-comparison}).

\leadtag{Cost and liveness}{tagsetup}{\astral spends tokens and liveness to keep false acceptance low.}
On the code-patching domain at $n{=}7$, a decision costs 8.1K tokens under MV, 16.4K under CP-WBFT, and 12.0K under \astral (the cost table in Appendix~\ref{app:extra}).
At $n{=}31$ the costs are 36.9K, 180.0K, and 172.7K, and on the same domain MV's attack success under A4 is 46.7\% against 0\% for \astral.
Under counter-spam (A5), 55.2\% of decisions end as \texttt{DISPUTED} at $n{=}7$ and 63.3\% at $n{=}31$, independent of the per-assessor counter budget (\textbf{Appendix~\ref{app:discussion:disputed}}).
The stable-finality rate under attacks A1--A4 is 43.9\% at $n{=}7$, so more than half of the attacked verdicts are flagged for audit.

\takeawaybox{\astral fails conservatively. Its residual risk stays small when assessors are diverse, and under attack \astral trades liveness for safety by flagging more verdicts as \texttt{DISPUTED}.}

\leadtag{Limitations}{tagthreat}{Six boundaries apply to these results.}
MFV is synthetic, and SciFact and FEVER are static corpora.
The live CVE cohort of 80 claims is the only evaluation with mutable Web evidence, and it evaluates \astral without baselines.
The bound is distributional and gives no guarantee against adaptive adversaries who model every assessor.
Content that steers more than $f$ assessors to the same wrong label lies outside the quorum guarantee and appears only through $\epsilon$ and $\rho_{k_h}$ (\S\ref{sec:threat:faults}).
\astral bounds risk conditional on the committed evidence, so evidence that retrieval never collected is beyond its scope.
The evaluated Byzantine assessors do not withhold \texttt{DA\_ACK} to stall $\daqc$, and latency is measured only in logical rounds.
Assessor diversity is self-declared in our setting, and \textbf{Appendix~\ref{app:discussion}} discusses attested diversity and other deployment questions.


==> tables/generated_tables.tex <==
\begin{table*}[t]
\centering
\caption{Attack Success Rate (\textbf{ASR}, \%, $\downarrow$) across attack vectors. Clopper--Pearson 95\% CI.}\label{tab:asr}
\small
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{@{}llccccc@{}}
\toprule
\textbf{Attack} & \textbf{Domain} & \textbf{Oracle} & \textbf{L1-BFT} & \textbf{MV} & \textbf{CP-WBFT} & \textbf{\astral} \\
\midrule
\multicolumn{7}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 36.0~[22.9,\,50.8] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 26.0~[14.6,\,40.3] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 6.7~[0.8,\,22.1] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 20.0~[6.8,\,40.7] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 20.0~[10.0,\,33.7] & 4.0~[0.5,\,13.7] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 12.0~[2.5,\,31.2] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 28.0~[16.2,\,42.5] & 4.0~[0.5,\,13.7] \\
\midrule
\multicolumn{7}{c}{\emph{Panel B: $n = 13$, $f = 4$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 20.0~[7.7,\,38.6] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 32.0~[14.9,\,53.5] & 32.0~[14.9,\,53.5] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 36.0~[22.9,\,50.8] & 4.0~[0.5,\,13.7] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 20.0~[6.8,\,40.7] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 26.0~[14.6,\,40.3] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 24.0~[9.4,\,45.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 22.0~[11.5,\,36.0] & 4.0~[0.5,\,13.7] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 28.0~[12.1,\,49.4] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 30.0~[17.9,\,44.6] & 2.0~[0.1,\,10.6] \\
\midrule
\multicolumn{7}{c}{\emph{Panel C: $n = 31$, $f = 10$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 36.7~[19.9,\,56.1] & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 52.0~[31.3,\,72.2] & 24.0~[9.4,\,45.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 34.0~[21.2,\,48.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 28.0~[16.2,\,42.5] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 14.0~[5.8,\,26.7] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 13.3~[3.8,\,30.7] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 32.0~[14.9,\,53.5] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 38.0~[24.7,\,52.8] & 4.0~[0.5,\,13.7] \\
\midrule
\multicolumn{7}{c}{\emph{Panel D: $n = 67$, $f = 22$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 40.0~[22.7,\,59.4] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 80.0~[59.3,\,93.2] & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 36.0~[22.9,\,50.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 6.7~[0.8,\,22.1] & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 26.0~[14.6,\,40.3] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 13.3~[3.8,\,30.7] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 16.0~[7.2,\,29.1] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 38.0~[24.7,\,52.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multicolumn{7}{c}{\emph{Panel E: $n = 100$, $f = 33$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 26.7~[12.3,\,45.9] & 6.7~[0.8,\,22.1] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 72.0~[50.6,\,87.9] & 24.0~[9.4,\,45.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 34.0~[21.2,\,48.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 28.0~[16.2,\,42.5] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 16.0~[7.2,\,29.1] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 13.3~[3.8,\,30.7] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 32.0~[14.9,\,53.5] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 36.0~[22.9,\,50.8] & \textbf{0.0~[0.0,\,7.1]} \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table}[t]
\centering
\caption{Semantic Correctness Success Rate (\textbf{SCSR}, \%, $\uparrow$) on benign inputs.}\label{tab:scsr}
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Domain} & \textbf{Oracle} & \textbf{L1-BFT} & \textbf{MV} & \textbf{CP-WBFT} & \textbf{\astral} \\
\midrule
\multicolumn{6}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
CVP & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} \\
SLA & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 98.0 \\
MFV & \textbf{100.0} & 50.0 & 87.0 & 88.0 & 86.0 \\
\midrule
\multicolumn{6}{c}{\emph{Panel B: $n = 13$, $f = 4$}} \\
\midrule
CVP & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 88.3 \\
SLA & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 70.0 \\
MFV & \textbf{100.0} & 50.0 & 87.0 & 88.0 & 85.0 \\
\midrule
\multicolumn{6}{c}{\emph{Panel C: $n = 31$, $f = 10$}} \\
\midrule
CVP & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 88.3 \\
SLA & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 70.0 \\
MFV & \textbf{100.0} & 50.0 & 87.0 & 88.0 & 85.0 \\
\midrule
\multicolumn{6}{c}{\emph{Panel D: $n = 67$, $f = 22$}} \\
\midrule
CVP & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 88.3 \\
SLA & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 70.0 \\
MFV & \textbf{100.0} & 50.0 & 87.0 & 88.0 & 85.0 \\
\midrule
\multicolumn{6}{c}{\emph{Panel E: $n = 100$, $f = 33$}} \\
\midrule
CVP & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 88.3 \\
SLA & \textbf{100.0} & 50.0 & \textbf{100.0} & \textbf{100.0} & 70.0 \\
MFV & \textbf{100.0} & 50.0 & 87.0 & 88.0 & 85.0 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{\astral{} accountability metrics by attack vector.}\label{tab:accountability}
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Metric} & \textbf{Attack~1} & \textbf{Attack~2} & \textbf{Attack~3} & \textbf{Attack~4} \\
\midrule
\multicolumn{5}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
Protocol Correctness (\%, $\uparrow$) & 91.9 & 92.9 & 92.9 & 92.4 \\
Detection Latency (rounds, $\downarrow$) & 1.0 & 1.0 & 1.0 & 1.0 \\
Protocol Error Rate (\%, $\downarrow$) & 8.1 & 7.1 & 7.1 & 7.6 \\
$\vstruct$ Rejection Rate (\%) & 0.0 & 0.0 & 0.0 & 0.0 \\
Counter-Card Filing Rate (\%) & 59.0 & 58.6 & 56.7 & 59.0 \\
$\crqc$ Triage Resolution (\%) & 5.6 & 5.7 & 5.0 & 8.9 \\
\texttt{DISPUTED} Fallback Rate (\%) & 55.7 & 55.2 & 53.8 & 53.8 \\
\midrule
\multicolumn{5}{c}{\emph{Panel B: $n = 31$, $f = 10$}} \\
\midrule
Protocol Correctness (\%, $\uparrow$) & 92.4 & 86.7 & 88.6 & 92.4 \\
Detection Latency (rounds, $\downarrow$) & 1.0 & 1.0 & 1.0 & 1.0 \\
Protocol Error Rate (\%, $\downarrow$) & 7.6 & 13.3 & 11.4 & 7.6 \\
$\vstruct$ Rejection Rate (\%) & 0.0 & 0.0 & 0.0 & 0.0 \\
Counter-Card Filing Rate (\%) & 63.3 & 73.3 & 68.1 & 63.3 \\
$\crqc$ Triage Resolution (\%) & 10.5 & 16.2 & 12.6 & 14.3 \\
\texttt{DISPUTED} Fallback Rate (\%) & 56.7 & 61.4 & 59.5 & 54.3 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{Post-hoc accountability comparison across protocols. Attacks~1--3, all domains. N/A: protocol lacks the structural mechanism.}\label{tab:accountability-comparison}
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Metric} & \textbf{MV} & \textbf{CP-WBFT} & \textbf{\astral} \\
\midrule
\multicolumn{4}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
Protocol Correctness (\%, $\uparrow$) & 93.3 & 90.0 & 92.5 \\
Byzantine Detection Rate (\%, $\uparrow$) & N/A & N/A & 58.1 \\
$\crqc$ Triage Resolution (\%) & N/A & N/A & 5.5 \\
Finality Certificate (\texttt{StableQC}, \%) & N/A & N/A & 43.8 \\
\midrule
\multicolumn{4}{c}{\emph{Panel B: $n = 31$, $f = 10$}} \\
\midrule
Protocol Correctness (\%, $\uparrow$) & 90.3 & 90.5 & 89.2 \\
Byzantine Detection Rate (\%, $\uparrow$) & N/A & N/A & 68.3 \\
$\crqc$ Triage Resolution (\%) & N/A & N/A & 13.3 \\
Finality Certificate (\texttt{StableQC}, \%) & N/A & N/A & 39.8 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{Security--correctness profile (A1--A4, all domains). Attack Rejection Rate $= 100 - \text{ASR}$; Benign Correctness $=$ SCSR; Decision Margin measures how strongly the protocol favoured false-accept on failed trials ($\downarrow$). Bottom three metrics are structural to \astral.}\label{tab:protocol-comparison}
\small
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Metric} & \textbf{L1-BFT} & \textbf{MV} & \textbf{CP-WBFT} & \textbf{\astral} \\
\midrule
\multicolumn{5}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
Attack Rejection Rate (\%, $\uparrow$) & 0.0 & 96.9 & 82.1 & \textbf{98.6} \\
Benign Correctness (SCSR \%, $\uparrow$) & 50.0 & 93.8 & \textbf{94.3} & 92.9 \\
Decision Margin ($\downarrow$) & +0.286 & +0.495 & +0.573 & \textbf{+0.071} \\
\midrule
Byzantine Detection Rate (\%) & --- & --- & --- & 58.3 \\
$\crqc$ Resolution (\%) & --- & --- & --- & 6.3 \\
Finality Certificate (\%) & --- & --- & --- & 43.9 \\
\midrule
\multicolumn{5}{c}{\emph{Panel B: $n = 31$, $f = 10$}} \\
\midrule
Attack Rejection Rate (\%, $\uparrow$) & 0.0 & 81.7 & 79.5 & \textbf{99.0} \\
Benign Correctness (SCSR \%, $\uparrow$) & 50.0 & 93.8 & \textbf{94.3} & 82.4 \\
Decision Margin ($\downarrow$) & +0.323 & \textbf{+0.202} & +0.445 & +0.226 \\
\midrule
Byzantine Detection Rate (\%) & --- & --- & --- & 67.0 \\
$\crqc$ Resolution (\%) & --- & --- & --- & 13.5 \\
Finality Certificate (\%) & --- & --- & --- & 41.0 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation: ASR (\%) under A2 (Cascading Hallucination).}\label{tab:ablation}
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{CVP}} & \multicolumn{2}{c}{\textbf{MFV}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Configuration} & \textbf{ASR$\downarrow$} & \textbf{$\Delta$} & \textbf{ASR$\downarrow$} & \textbf{$\Delta$} \\
\midrule
\multicolumn{5}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
L1-BFT (no semantic layer) & 100.0 & --- & 100.0 & --- \\
+ $\vstruct$ + $\vinfer$ ($\semqc$) & 0.0 & $-$100.0 & 6.0 & $-$94.0 \\
+ Full \astral ($\crqc$ triage) & \textbf{0.0} & $-$0.0 & \textbf{2.0} & $-$4.0 \\
\astral-NoDiv (same model) & 0.0 & --- & 2.0 & --- \\
Simple Threshold (single agent) & 0.0 & --- & 2.0 & --- \\
Oracle Ceiling & 0.0 & --- & 0.0 & --- \\
\midrule
\multicolumn{5}{c}{\emph{Panel B: $n = 31$, $f = 10$}} \\
\midrule
L1-BFT (no semantic layer) & 100.0 & --- & 100.0 & --- \\
+ $\vstruct$ + $\vinfer$ ($\semqc$) & 0.0 & $-$100.0 & 4.0 & $-$96.0 \\
+ Full \astral ($\crqc$ triage) & \textbf{0.0} & $-$0.0 & \textbf{2.0} & $-$2.0 \\
\astral-NoDiv (same model) & 0.0 & --- & 2.0 & --- \\
Simple Threshold (single agent) & 0.0 & --- & 2.0 & --- \\
Oracle Ceiling & 0.0 & --- & 0.0 & --- \\
\bottomrule
\end{tabular}
}
\end{table}



\begin{table}[t]
\centering
\caption{Correlation factor $\rho_{k_h}$ at $\tau = 0.7$, MFV domain (most correlation-sensitive).}\label{tab:rho}
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Diversity Config} & \textbf{$k_h$} & \textbf{$\Pr[\cap A_i]$} & \textbf{$\epsilon^{k_h}$} & \textbf{$\rho_{k_h}$} \\
\midrule
Same model family & 2 & $2.0 \times 10^{-2}$ & $4.0 \times 10^{-4}$ & 50.0 \\
Mixed 2 families & 2 & $2.0 \times 10^{-2}$ & $9.0 \times 10^{-4}$ & 22.2 \\
Mixed 3 families & 3 & $0$ & $3.7 \times 10^{-5}$ & 0.0 \\
Full diversity (4 families) & 4 & $0$ & $1.5 \times 10^{-6}$ & 0.0 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{Effective semantic failure rate $\hat{\delta}$. $\tau = 0.7$, MFV domain.}\label{tab:delta}
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Configuration} & \textbf{$\hat{\delta}$ ($\downarrow$)} & \textbf{$\hat{p}_{\mathit{ch}}$ ($\uparrow$)} & \textbf{Bound $\delta$ ($\downarrow$)} \\
\midrule
$\vinfer$ only, same model & $2.0 \times 10^{-2}$ & --- & $2.0 \times 10^{-2}$ \\
$\vinfer$ only, full diversity & $< 10^{-5}$ & --- & $< 10^{-5}$ \\
Full \astral, full diversity & $< 10^{-5}$ & 0.57 & $< 10^{-5}$ \\
Full \astral, full div.\ + det.\ proofs & $< 10^{-5}$ & 0.87 & $< 10^{-5}$ \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/tab_asr.tex <==
\begin{table*}[t]
\centering
\caption{Attack Success Rate (\textbf{ASR}, \%, $\downarrow$) across attack vectors. Clopper--Pearson 95\% CI.}\label{tab:asr}
\evaltablefont
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{@{}llccccc@{}}
\toprule
\textbf{Attack} & \textbf{Domain} & \textbf{Oracle} & \textbf{L1-BFT} & \textbf{MV} & \textbf{CP-WBFT} & \textbf{\astral} \\
\midrule
\multicolumn{7}{c}{\emph{Panel A: $n = 7$, $f = 2$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 36.0~[22.9,\,50.8] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 26.0~[14.6,\,40.3] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 6.7~[0.8,\,22.1] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 20.0~[6.8,\,40.7] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 20.0~[10.0,\,33.7] & 4.0~[0.5,\,13.7] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 12.0~[2.5,\,31.2] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 28.0~[16.2,\,42.5] & 4.0~[0.5,\,13.7] \\
\midrule
\multicolumn{7}{c}{\emph{Panel B: $n = 13$, $f = 4$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 20.0~[7.7,\,38.6] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 32.0~[14.9,\,53.5] & 32.0~[14.9,\,53.5] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 36.0~[22.9,\,50.8] & 4.0~[0.5,\,13.7] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 20.0~[6.8,\,40.7] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 26.0~[14.6,\,40.3] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 24.0~[9.4,\,45.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 22.0~[11.5,\,36.0] & 4.0~[0.5,\,13.7] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 28.0~[12.1,\,49.4] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 30.0~[17.9,\,44.6] & 2.0~[0.1,\,10.6] \\
\midrule
\multicolumn{7}{c}{\emph{Panel C: $n = 31$, $f = 10$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 36.7~[19.9,\,56.1] & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 52.0~[31.3,\,72.2] & 24.0~[9.4,\,45.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 34.0~[21.2,\,48.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 28.0~[16.2,\,42.5] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & \textbf{0.0~[0.0,\,11.6]} & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 14.0~[5.8,\,26.7] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 13.3~[3.8,\,30.7] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 32.0~[14.9,\,53.5] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 38.0~[24.7,\,52.8] & 4.0~[0.5,\,13.7] \\
\midrule
\multicolumn{7}{c}{\emph{Panel D: $n = 67$, $f = 22$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 40.0~[22.7,\,59.4] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 80.0~[59.3,\,93.2] & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 36.0~[22.9,\,50.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 6.7~[0.8,\,22.1] & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 26.0~[14.6,\,40.3] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 13.3~[3.8,\,30.7] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 16.0~[7.2,\,29.1] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 38.0~[24.7,\,52.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multicolumn{7}{c}{\emph{Panel E: $n = 100$, $f = 33$}} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A1: Prompt\\Injection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 26.7~[12.3,\,45.9] & 6.7~[0.8,\,22.1] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 72.0~[50.6,\,87.9] & 24.0~[9.4,\,45.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 34.0~[21.2,\,48.8] & \textbf{0.0~[0.0,\,7.1]} \\
\midrule
\multirow{3}{*}{\shortstack[l]{A2: Cascading\\Hallucination}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 10.0~[2.1,\,26.5] & \textbf{0.0~[0.0,\,11.6]} & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 16.0~[4.5,\,36.1] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 8.0~[2.2,\,19.2] & 28.0~[16.2,\,42.5] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A3: Collusion \&\\Suppression}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 3.3~[0.1,\,17.2] & 3.3~[0.1,\,17.2] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & \textbf{0.0~[0.0,\,13.7]} & 8.0~[1.0,\,26.0] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 6.0~[1.3,\,16.5] & 16.0~[7.2,\,29.1] & 2.0~[0.1,\,10.6] \\
\midrule
\multirow{3}{*}{\shortstack[l]{A4: Adaptive\\Selection}}
& CVP & \textbf{0.0~[0.0,\,11.6]} & 100.0~[88.4,\,100.0] & 46.7~[28.3,\,65.7] & 13.3~[3.8,\,30.7] & \textbf{0.0~[0.0,\,11.6]} \\
& SLA & \textbf{0.0~[0.0,\,13.7]} & 100.0~[86.3,\,100.0] & 88.0~[68.8,\,97.5] & 32.0~[14.9,\,53.5] & \textbf{0.0~[0.0,\,13.7]} \\
& MFV & \textbf{0.0~[0.0,\,7.1]} & 100.0~[92.9,\,100.0] & 10.0~[3.3,\,21.8] & 36.0~[22.9,\,50.8] & \textbf{0.0~[0.0,\,7.1]} \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/tab_multiseed.tex <==
\begin{table}[t]
\centering
\caption{Pooled ASR over five seeds (mean $\pm$ std). \astral{} remains best at every committee size.}\label{tab:multiseed}
\evaltablefont
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Protocol} & \textbf{$n{=}7$} & \textbf{$n{=}13$} & \textbf{$n{=}31$} & \textbf{$n{=}67$} & \textbf{$n{=}100$} \\
\midrule
\astral   & \astralcell{$1.4 \pm 0.2$} & \astralcell{$1.1 \pm 0.2$} & \astralcell{$1.1 \pm 0.1$} & \astralcell{$0.5 \pm 0.1$} & \astralcell{$0.5 \pm 0.0$} \\
MV        & $2.9 \pm 0.3$          & $17.2 \pm 0.8$         & $18.8 \pm 0.4$         & $20.5 \pm 0.6$         & $20.2 \pm 0.7$ \\
CP-WBFT   & $18.6 \pm 0.4$         & $21.7 \pm 0.8$         & $14.9 \pm 1.1$         & $21.0 \pm 0.8$         & $20.7 \pm 0.4$ \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/tab_ratelimit.tex <==
\begin{table}[t]
\centering
\caption{Counter-spam ablation for A5. DISPUTED is invariant in $K$, implicating triage \texttt{SUSTAIN} votes rather than counter volume.}\label{tab:ratelimit}
\evaltablefont
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{$n$} & \textbf{$K$} & \textbf{Counters/trial} & \textbf{DISPUTED (\%)} & \textbf{Sustained/trial} \\
\midrule
\multirow{3}{*}{7}  & 0 (PoW)        & 2.7   & \astralsoft{55.2} & 2.2 \\
                    & 1 (rate-limit) & 4.7   & \astralsoft{55.2} & 2.2 \\
                    & $f$ (vanilla)  & 6.7   & \astralsoft{55.2} & 2.2 \\
\midrule
\multirow{3}{*}{31} & 0 (PoW)        & 11.4  & \astralsoft{63.3} & 7.7 \\
                    & 1 (rate-limit) & 21.4  & \astralsoft{63.3} & 7.7 \\
                    & $f$ (vanilla)  & 111.4 & \astralsoft{63.3} & 7.7 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/tab_realbench.tex <==
\begin{table}[t]
\centering
\caption{\astral{} on SciFact and FEVER at $n{=}7$, $f{=}2$ with a heterogeneous 7-model committee. SCSR is benign correctness; ASR is reported under A1--A4 with pooled 95\% CI.}\label{tab:realbench}
\evaltablefont
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Protocol} & \textbf{SCSR} & \textbf{A1} & \textbf{A2} & \textbf{A3} & \textbf{A4} & \makecell[c]{\textbf{Pool ASR}\\\textbf{[95\% CI]}} \\
\midrule
\multicolumn{7}{c}{\emph{SciFact}} \\
\midrule
Oracle$^{\dagger}$ & 100.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\,[0.0,0.9] \\
L1-BFT & 50.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\,[99.1,100.0] \\
MV & 92.5 & 9.0 & 5.0 & 5.0 & 12.0 & 7.8\,[5.3,10.8] \\
CP-WBFT & 92.0 & 13.0 & 7.0 & 33.0 & 28.0 & 20.2\,[16.4,24.5] \\
\astral & \astralsoft{86.5} & \astralcell{0.0} & \astralcell{0.0} & \astralcell{0.0} & \astralcell{0.0} & \astralcell{0.0\,[0.0,0.9]} \\
\cmidrule(l){1-7}
Simple-Thr. & 88.5 & 4.0 & 4.0 & 0.0 & 4.0 & 3.0\,[1.6,5.2] \\
\astral-NoDiv & 88.5 & 4.0 & 4.0 & 0.0 & 4.0 & 3.0\,[1.6,5.2] \\
\astral-NoCh & \astralsoft{93.5} & \astralsoft{2.0} & \astralsoft{1.0} & \astralsoft{0.0} & \astralsoft{4.0} & \astralsoft{1.8\,[0.7,3.6]} \\
\midrule
\multicolumn{7}{c}{\emph{FEVER}} \\
\midrule
Oracle$^{\dagger}$ & 100.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\,[0.0,0.9] \\
L1-BFT & 50.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\,[99.1,100.0] \\
MV & 96.5 & 5.0 & 3.0 & 3.0 & 5.0 & 4.0\,[2.3,6.4] \\
CP-WBFT & 97.0 & 3.0 & 3.0 & 3.0 & 4.0 & 3.2\,[1.7,5.5] \\
\astral & \astralsoft{94.5} & \astralcell{0.0} & \astralcell{0.0} & \astralcell{0.0} & \astralcell{2.0} & \astralcell{0.5\,[0.1,1.8]} \\
\cmidrule(l){1-7}
Simple-Thr. & 95.5 & 3.0 & 2.0 & 3.0 & 3.0 & 2.8\,[1.4,4.9] \\
\astral-NoDiv & 95.5 & 3.0 & 2.0 & 3.0 & 3.0 & 2.8\,[1.4,4.9] \\
\astral-NoCh & \astralsoft{96.5} & \astralsoft{3.0} & \astralsoft{1.0} & \astralsoft{2.0} & \astralsoft{4.0} & \astralsoft{2.5\,[1.2,4.5]} \\
\bottomrule
\multicolumn{7}{l}{\evaltablenotefont $^{\dagger}$Oracle = upper-bound ceiling. Committee spans 7 distinct model families.} \\
\end{tabular}
}
\end{table}


==> tables/www_mfv_asr.tex <==
\begin{table}[t]
\centering
\caption{Attack success rate (\%, lower is better) on MFV multi-source claims. Panel A varies the attack at $n{=}7$, and Panel B varies committee size under model-aware corruption (A4). Each cell has 50 refuted claims.}
\label{tab:mfv_asr}
\resizebox{\ifdim\width>\columnwidth\columnwidth\else\width\fi}{!}{%
\begin{tabular}{@{}c@{\hspace{8pt}}c@{}}
\begin{tabular}{@{}lcccc@{}}
\multicolumn{5}{c}{\textbf{A. Attacks at $n{=}7$}}\\[1pt]
\toprule
\textbf{Protocol} & \textbf{A1} & \textbf{A2} & \textbf{A3} & \textbf{A4} \\
\midrule
MV & 6.0 & 6.0 & 8.0 & 6.0 \\
CP-WBFT & 36.0 & 26.0 & 20.0 & 28.0 \\
\astral & \astralcell{2.0} & \astralcell{2.0} & \astralcell{4.0} & \astralcell{4.0} \\
\bottomrule
\end{tabular}
&
\begin{tabular}{@{}lccccc@{}}
\multicolumn{6}{c}{\textbf{B. A4 across committee size $n$}}\\[1pt]
\toprule
\textbf{Protocol} & \textbf{7} & \textbf{13} & \textbf{31} & \textbf{67} & \textbf{100} \\
\midrule
MV & 6.0 & 10.0 & 10.0 & 10.0 & 10.0 \\
CP-WBFT & 28.0 & 30.0 & 38.0 & 38.0 & 36.0 \\
\astral & \astralcell{4.0} & \astralcell{2.0} & \astralcell{4.0} & \astralcell{0.0} & \astralcell{0.0} \\
\bottomrule
\end{tabular}
\end{tabular}%
}
\end{table}


==> tables/www_nonweb_asr.tex <==
\begin{table}[!htbp]
\centering
\caption{\looseness=-1 Attack success rate (\%, lower is better) on two non-Web domains under model-aware corruption (A4) by committee size $n$. Cells cover 25 (SLA) or 30 (CVP) refuted items.}
\label{tab:nonweb_asr}
\resizebox{\ifdim\width>\columnwidth\columnwidth\else\width\fi}{!}{%
\begin{tabular}{@{}c@{\hspace{8pt}}c@{}}
\begin{tabular}{@{}lccccc@{}}
\multicolumn{6}{c}{\textbf{A. Log auditing (SLA), A4}}\\[1pt]
\toprule
\textbf{Protocol} & \textbf{7} & \textbf{13} & \textbf{31} & \textbf{67} & \textbf{100} \\
\midrule
MV & {0.0} & {88.0} & {88.0} & {88.0} & {88.0} \\
CP-WBFT & {12.0} & {28.0} & {32.0} & {16.0} & {32.0} \\
\textbf{\astral} & {\textbf{0.0}} & {\textbf{0.0}} & {\textbf{0.0}} & {\textbf{0.0}} & {\textbf{0.0}} \\
\bottomrule
\end{tabular}
&
\begin{tabular}{@{}lccccc@{}}
\multicolumn{6}{c}{\textbf{B. Code patching (CVP), A4}}\\[1pt]
\toprule
\textbf{Protocol} & \textbf{7} & \textbf{13} & \textbf{31} & \textbf{67} & \textbf{100} \\
\midrule
MV & {0.0} & {46.7} & {46.7} & {46.7} & {46.7} \\
CP-WBFT & {0.0} & {3.3} & {13.3} & {10.0} & {13.3} \\
\textbf{\astral} & {\textbf{0.0}} & {\textbf{0.0}} & {\textbf{0.0}} & {\textbf{0.0}} & {\textbf{0.0}} \\
\bottomrule
\end{tabular}
\end{tabular}%
}
\end{table}

